The Age-Dependent Vertical Actions of Young Stars in the Galaxy

Stars in the Galactic disk are born on cold, nearly circular orbits with small vertical excursions. After their birth, their orbits evolve, driven by small- or large-scale perturbations in the Galactic disk's gravitational potential. Here, we study the vertical motions of young stars over their first few orbital periods, using a sample of OBA stars from \textit{Gaia} E/DR3, which includes radial velocities and ages $\tau$ from LAMOST. We constructed a parametric model for the time evolution of the stellar orbits' mean vertical actions $J_z$ as a function of Galactocentric radius, $R_{\mathrm{GC}}$. Accounting for data uncertainties, we use Markov Chain Monte Carlo (MCMC) analysis in annuli of Galactocentric radius to constrain the model parameters. Our best-fit model shows a remarkably linear increase of vertical actions with age across all Galactocentric radii examined. Orbital \textit{heating} by random scattering could offer a straightforward interpretation for this trend. However, various other dynamical aspects of the Galactic disk, such as stars being born in a warped disk, might offer alternative explanations that could be tested in the future.

==> graphical_model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% The caption of this graphical model
% is at the bottom of the page
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{shapes,arrows,positioning,fit}

\begin{figure*}
\centering
%
% Start the graphical model
%
\begin{tikzpicture}[->,>=stealth']


% define colors
\definecolor{bblue}{RGB}{34,94,168}
\definecolor{ggreen}{RGB}{35,132,67}
\definecolor{rm}{RGB}{140,45,4}

%---------------------------------------
% Make some commands
%---------------------------------------
\tikzstyle{main}=[circle, minimum size = 12mm, line width=0.4mm, draw =black!80, node distance = 7mm]
\tikzstyle{ellip}=[ellipse, minimum width=20mm, minimum height=12mm), line width=0.4mm, draw =black!80, node distance = 7mm]
\tikzstyle{err}=[circle, minimum size = 2mm, thick, draw =black!100, node distance = 9mm]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{box}=[rectangle, draw=black!100]
\tikzstyle{line}=[draw]

%-----------------------------------------
% Make Nodes
%-----------------------------------------
   % 0th floor = observables
   \node[ellip, minimum width=7mm, fill = black!15] (xv) [label={[align=center]center:$R_i$\\ $z_i$}] { };
   \node[ellip, minimum width=7mm, fill=black!15] (v) [left=of xv][label={[align=center]center:$v_{Ri}$\\ $v_{\phi i}$}] { };
   \node[ellip, minimum width=15mm,fill = black!15] (feobs) [right=of xv, label=center:{[Fe/H]$_{\mathrm{obs}i}$}] { };
   \node[main, fill = black!15] (tobs) [right=of feobs, label=center:$\tau_{\mathrm{obs}i}$] { };
   \node[ellip, minimum width=28mm, fill = black!15] (evol) [right=of tobs][draw, align=center] {Evolutionary  \\stage $i$ };
   
   % 1st floor: action and metallicity
   \node[main, fill=white!100](J)[above=of xv, label=center:{$\boldsymbol{J}_i, \boldsymbol{\theta}_i$}] {};
   \node[main, fill=white!100](fe)[above=of feobs, label=center:{[Fe/H]$_i$}] {};
   
   % 2nd floor: birth conditions: birth angular momentum, age
   \node[main, fill=white!100](Lz0)[above=of J, label=center:{$L_{z0i}$}] {};
   \node[main, fill=white!100](t)[above=26mm of tobs, label=center:{$\tau_i$}] {};

   % 3rd floor: birth parameters
   \node[ellip, fill=white!100](Rd0)[above=of Lz0][draw=ggreen, line width=0.8mm, align=center]{Formation\\ structure, $R_{d0}$};   
 %  \node[ellip, fill = white!100](SFH)[above=of t, label=right:{Star formation history $\tau_\mathrm{SFR}, x$}][draw=ggreen, line width=0.8mm] {};
   \node[ellip, fill=white!100](SFH)[above=of t][draw=ggreen, line width=0.8mm, align=center]{Star formation \\history, $\tau_\mathrm{SFR}, x$};

   % Left:  Potential and secular evolution
   \node[ellip, minimum width=25mm, fill=white!100](secular)[left=20mm of J][draw=rm, align=center, line width=0.8mm]{Secular \\ evolution\\$\sigma_{Lz}$, $\sigma_{vR0}$, \\$R_\mathrm{dheating}$, $\beta$}; 
   \node[err, fill=black!100](vert)[left=20mm of Lz0, label={[align=center]left:Vertical\\ heating}]{};  
   %\node[err, fill=black!100](pot)[left=20mm of Lz0, label=left:$\Phi_\mathrm{pot}$] {};   
   
   % Right: chemical enrichment
   \node[ellip, minimum width=25mm, fill=white!100, draw=bblue, line width=0.8mm](chemical)[right=65mm of fe][draw, align=center]{Chemical \\ enrichment \\$\gamma_\mathrm{[Fe/H]}$ \\ $\mathrm{[Fe/H]_{max}}$ \\ $\mathrm{\nabla\mathrm{[Fe/H]}}$};
   
   % errors
   \node[err, fill=black!100](errdyn)[left=of v, label=below:$\sigma_{v}$] {}; 
   \node[err, fill=black!100](errfe)[below=of feobs, label=below:$\sigma_{[\mathrm{Fe}/\mathrm{H}]}$] {}; 
   \node[err, fill=black!100](errt)[below=of tobs, label=below:$\sigma_{\tau}$] {};
   
   % selection function
   \node[err, fill=black!100](selfunc)[below=of xv, label={[align=center]below: APOGEE \\spatial selection}]{};
   \node[err, fill=black!100](RC)[below=of evol, label={[align=center]below: Red Clump\\ selection}]{};
   
   % Potential
   \node[err, fill=black!100](pot)[left=11mm of selfunc, label=left:$\Phi_\mathrm{pot}$] {};

   % Rectangle around single objects to take the product over
   \node[rectangle, fit=(v) (Lz0)(evol), label=above right:{$ i=1,...,N $}] (rect) {};
   \node[rectangle, fit=(rect), inner sep=4.5mm, draw=black!100] {};

%------------------------------------------------
% Draw the connections
%------------------------------------------------
  \path (Rd0) edge [connect] (Lz0)
		(Lz0) edge [connect] (t)
		(SFH) edge [connect] (t)
		(pot) edge [connect] (v)
		(pot) edge [connect] (xv)
		(Lz0) edge [connect] (J)
		(Lz0) edge [connect] (fe)
		(t) edge [connect] (J)
		(t) edge [connect] (fe)
		(t) edge [connect] (evol)
		(t) edge [connect] (tobs)
		(secular) edge [connect] (J)
		(vert) edge [connect] (J)
		(J) edge [connect] (xv)
		(J) edge [connect] (v)
		%(xv) edge[bend right] node [left] {} (v)
		%(v) edge[bend left=-20] node [right] {} (xv)
		%(xv) edge [connect] (v)
		(fe) edge [connect] (feobs)
		(chemical) edge [connect] (fe)
		(errdyn) edge [connect] (v)
		(errfe) edge [connect] (feobs)
		(errt) edge [connect] (tobs)
		(selfunc) edge [connect] (xv)
		(RC) edge [connect] (evol);
\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CAPTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig_graphical_model} Simplified probabilistic graphical model for the joint distribution $p(\mathbf{x_i}, \mathbf{v_i}, \fe_i, \tau_\mathrm{obsi}\} ~|~ \ppm)$ 
for APOGEE data set. This is the product of a global model for the Milky Way disk and of APOGEE selection function, marginalized over a model for data uncertainties. 
The circles filled in gray contain the observables to model, i.e. APOGEE red clump stars. 
The circles inside the large rectangle contain model variables: the true birth angular momentum, true age, true action vector, true metallicity. 
The ellipses outside the rectangle contain the model parameters to fit: scale length at birth, star formation time-scale, inside-out parameter, 
secular evolution parameters and chemical enrichment parameters. The black points are fixed aspects of the model: present-day potential of the Milky Way, 
noise model and APOGEE selection function.}
\end{figure*}


==> graphical_model_dyn.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% To do: zoom in the action part?
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centering
%
% Start the graphical model
%
\begin{tikzpicture}


% define colors
\definecolor{bblue}{RGB}{34,94,168}
\definecolor{ggreen}{RGB}{35,132,67}
\definecolor{rm}{RGB}{140,45,4}

%---------------------------------------
% Make some commands
%---------------------------------------
\tikzstyle{main}=[circle, minimum size = 12mm, line width=0.4mm, draw =black!80, node distance = 10mm]
\tikzstyle{ellip}=[ellipse, minimum width=24mm, minimum height=12mm), line width=0.4mm, draw =black!80, node distance = 10mm]
\tikzstyle{err}=[circle, minimum size = 2mm, thick, draw =black!100, node distance = 10mm]
\tikzstyle{connect}=[-latex, thick]
\tikzstyle{box}=[rectangle, draw=black!100]
\tikzstyle{line}=[draw]

%-----------------------------------------
% Make Nodes
%-----------------------------------------
   % 0th floor = observables
   \node[main, fill = black!15] (xv) [label=center:{$\mathbf{x}, \mathbf{v}$}] { };
   \node[ellip, minimum width=15mm,fill = black!15] (feobs) [right=of xv, label=center:{[Fe/H]$_\mathrm{obs}$}] { };
   \node[main, fill = black!15] (tobs) [right=of feobs, label=center:$\tau_\mathrm{obs}$] { };
   \node[ellip, minimum width=28mm, fill = black!15] (evol) [right=of tobs][draw, align=center] {Evolutionary  \\stage };
   
   % 1st floor: action and metallicity
   \node[main, fill=white!100](J)[above=of xv, label=center:{$\mathbf{J}$}] {};
   \node[main, fill=white!100](fe)[above=of feobs, label=center:{[Fe/H]}] {};
   
   % 2nd floor: birth conditions: birth angular momentum, age
   \node[main, fill=white!100](Lz0)[above=of J, label=center:{$L_{z0}$}] {};
   \node[main, fill=white!100](t)[above=32mm of tobs, label=center:{$\tau$}] {};

   % 3rd floor: birth parameters
   \node[ellip, fill=white!100](Rd0)[above=of Lz0][draw=ggreen, line width=0.8mm]{Formation structure $R_{d0}$};   
   \node[err, fill = black!100](SFH)[above=of t, label=right:{Star formation history $\tau_\mathrm{SFR}, x$}] {};

   % Left:  Potential and secular evolution
   \node[ellip, minimum width=25mm, fill=white!100](secular)[left=of J][draw=rm, align=center, line width=0.8mm]{Secular \\ evolution\\$\sigma_{Lz}$, $\sigma_{vR0}$, \\$R_\mathrm{dheating}$, $\beta$};   
   \node[err, fill=black!100](pot)[left=of Lz0, label=left:$\Phi_\mathrm{pot}$] {};   
   
   % Right: chemical enrichment
   \node[ellip, minimum width=25mm, fill=white!100, draw=bblue, line width=0.8mm](chemical)[right=72mm of fe][draw, align=center]{Chemical \\ enrichment \\$\gamma_\mathrm{[Fe/H]}$ \\ $\mathrm{[Fe/H]_{max}}$ \\ $\mathrm{\nabla\mathrm{[Fe/H]}}$};
   
   % errors
   \node[err, fill=black!100](errdyn)[left=of xv, label=below:$\sigma_{xv}$] {}; 
   \node[err, fill=black!100](errfe)[below=of feobs, label=below:$\sigma_{[Fe/H]}$] {}; 
   \node[err, fill=black!100](errt)[below=of tobs, label=below:$\sigma_{\tau}$] {}; 
   
   % selection function
   \node[err, fill=black!100](selfunc)[below=of xv, label={[align=center]below: APOGEE \\spatial selection}]{};
   \node[err, fill=black!100](RC)[below=of evol, label={[align=center]below: Red Clump\\ selection}]{};

   % Rectangle around single objects to take the product over
   \node[rectangle, fit=(Lz0)(evol), label=above right:{$ i=1,...,N $}] (rect) {};
   \node[rectangle, fit=(rect), inner sep=5mm, draw=black!100] {};

%------------------------------------------------
% Draw the connections
%------------------------------------------------
  \path (Rd0) edge [connect] (Lz0)
		(Lz0) edge [connect] (t)
		(SFH) edge [connect] (t)
		(pot) edge [connect] (J)
		(Lz0) edge [connect] (J)
		(Lz0) edge [connect] (fe)
		(t) edge [connect] (J)
		(t) edge [connect] (fe)
		(t) edge [connect] (evol)
		(t) edge [connect] (tobs)
		(secular) edge [connect] (J)
		(J) edge [connect] (xv)
		(fe) edge [connect] (feobs)
		(chemical) edge [connect] (fe)
		(errdyn) edge [connect] (xv)
		(errfe) edge [connect] (feobs)
		(errt) edge [connect] (tobs)
		(selfunc) edge [connect] (xv)
		(RC) edge [connect] (evol);
\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CAPTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig_graphical_model} Probabilistic graphical model for the joint distribution $p(\mathbf{x_i}, \mathbf{v_i}, \fe_i, \tau_\mathrm{obsi}\} ~|~ \ppm)$ for APOGEE data set. This is the product of a global model for the Milky Way disk and of APOGEE selection function, marginalized over a model for data uncertainties. The circles filled in gray contain the observables to model, i.e. APOGEE red clump stars. The circles inside the large rectangle contain model variables: the true birth angular momentum, true age, true action vector, true metallicity. The ellipses outside the rectangle contain the model parameters to fit: scale length at birth, secular evolution parameters and chemical enrichment parameters. The black points are fixed aspects of the model: star formation history, present-day potential of the Milky Way, noise model and APOGEE selection function.}
\end{figure}
